Towards Robust On-Ramp Merging via Augmented Multimodal Reinforcement Learning

Despite the success of AI-enabled onboard perception, on-ramp merging has been one of the main challenges for autonomous driving. Due to limited sensing range of onboard sensors, a merging vehicle can hardly observe main road conditions and merge properly. By leveraging the wireless communications between connected and automated vehicles (CAVs), a merging CAV has potential to proactively obtain the intentions of nearby vehicles. However, CAVs can be prone to inaccurate observations, such as the noisy basic safety messages (BSM) and poor quality surveillance images. In this paper, we present a novel approach for Robust on-ramp merge of CAVs via Augmented and Multi-modal Reinforcement Learning, named by RAMRL. Specifically, we formulate the on-ramp merging problem as a Markov decision process (MDP) by taking driving safety, comfort driving behavior, and traffic efficiency into account. To provide reliable merging maneuvers, we simultaneously leverage BSM and surveillance images for multi-modal observation, which is used to learn a policy model through proximal policy optimization (PPO). Moreover, to improve data efficiency and provide better generalization performance, we train the policy model with augmented data (e.g., noisy BSM and noisy surveillance images). Extensive experiments are conducted with Simulation of Urban MObility (SUMO) platform under two typical merging scenarios. Experimental results demonstrate the effectiveness and efficiency of our robust on-ramp merging design.

==> Chapters/Results_old.tex <==
In this section we first compare the results from training the environment with the BSM and Image data. 
\subsubsection{Training}
The merging vehicle is trained for 50000 steps. Fig \ref{fig:EpisodicRewards} shows the number of steps.The rewards are normalized between -10 to 10. 
We consider the following metrics to evaluate the merging vehicle performance \cite{RN11}.
\subsubsection{Testing}
Table \ref{tab:RewardPerState} shows the average of the total normalized rewards received by the ego vehicle in each episodes. The average is taken over 300 episodes and in each episode the total rewards is the sum of all the intermediate rewards the ego vehicle receives when tested on the trained policy.

\begin{table}[]
        \centering
        \begin{tabular}{ |p{2cm}|p{2cm}|p{2cm} |  }
        \hline
        \textbf{State}  & \textbf{Krauss Car \newline Following Model} & \textbf{Mean Rewards \newline Proposed Method}  \\ \hline
            Image & & \\ \hline  
            BSM & &\\ \hline
            Image + BSM & -0.359 & 8.065 \\ \hline
        \end{tabular}
        \caption{Average total rewards per episode}
        \label{tab:RewardPerState}
    \end{table}
\begin{enumerate}
    \item Average collision rate: Number of collisions per episodes.
    \item Traffic efficiency: Mean of velocities of the vehicles on the main road. This compares the impact of reward on the traffic efficiency. 
    \item compare diff PPO networks
    \item Success rate: compare completion of merging task for images, BSM vs images and BSM data. 
\end{enumerate}

==> Chapters/archive/Introduction.tex <==
% What are the problems in traffic why CAV is important , what are the developments in CAV or AV. 
There has been a substantial amount of research on the traffic flow, driving patterns, crashes and potential risks on road.
In a study on traffic accidents, NHTSA found human errors to be the major cause of traffic crashes on the road, other being environmental factors \cite{USDOT2015traffic}.  
%According to the statistics from the US Department of Transportation (USDOT) there is 7 billion miles of road travel each year, and about 2.7 million crashes occur during this travel \cite{USDOT2020traffic,USDOT2019traffic}. Human errors and adverse weather conditions are the critical reasons for accidents \cite{USDOT2015traffic}.
This can be avoided with vehicles capable of perception and decision making. Automakers and researchers have developed and tested different levels of automated vehicles over last few years. Some of these systems like advanced driver assistance systems (ADAS) have been successful to detect erroneous behavior of surrounding vehicles and take actions to avoid crash. However these systems use onboard sensors which have a limited sensing capability. On the contrary, Connected and automated vehicles (CAVs)  can communicate with each other to leverage the sensing capability of the surrounding vehicles to take accurate decisions in complex tasks. 

% How CAVs solve the traffic problem and why on ramp merging is complex and difficult task
Although CAVs vehicles have been able to achieve great success in some tasks, on-ramp merging is still a challenging task. To do a successful merge maneuver, the merging vehicle has to change the speed, select a gap between two vehicles and change the lane to merge.  Additionally, the merging vehicle has to cooperate with its surrounding vehicles and predict their behavior as well. Due to this on-ramp merging is a complex driving maneuver that requires a very high sensing ability and path planning. There are several proposed CAVs approaches that have been considered from the rule based algorithms, to supervised learning and reinforcement learning.

% what are the types of approaches and why use rl 
While rule-based algorithms are simpler to implement for a certain scenario, it is difficult to optimize to with increasing traffic flow. It is challenging to consider all the cases that the merging vehicle would encounter since the traffic flow is stochastic. The slot based approach \cite{urmson2008autonomous} determines the feasibility of merge based on gaps between the two vehicles. This approach and several other rule-based approaches are challenging to generalize in the real high traffic flow scenarios. Other popular approach is building the autonomous driving systems by using supervised machine learning algorithms. However, the supervised machine learning models have a disadvantage of covariant shift. This occurs when the distribution of training environment differs from the testing environment. Further, supervised machine learning requires a large number of training input data and labels. Collecting and labelling this large amount of data can be costly, time consuming and requires human interventions. Thus we propose to use reinforcement learning, a subset of artificial intelligence, in which the agent learns by interacting with the environment. We can thus collect large amount of data by interacting with the simulated environment and bridge the sim-to-real gap \cite{zhao2020sim}. 

% What is RL and why do we want to use it.

% Modality based classification 
Apart form the type of algorithm used, the type of modality is also important. For example the observed input information may come from various sensors which are prone to different types of noise. Most existing machine learning models use a single source of information for making decisions which can prove to unreliable in certain conditions. For example information from a single type of sensor-modality like a multi-camera setup may fail when driving in snow, dense fog or other adverse weather conditions. S. Chaturvedi \textit{et al.} \cite{chaturvedi2022pay} have discussed the need for multi-modal sensor fusion and designed a system for object detection when the input from one of the sensors is unreliable. 
%Designing a robust agent for successful merging maneuver when only partial information is available or when the information from the camera or the GPS data cannot be reliable is a challenging task. Given the above challenges, this paper proposes to leverage th

% What are contributions of this paper? 
We propose an End-to-End (E2E) model, one of the most common deep learning (DL) method, which takes the input data and outputs the control decisions directly. We first formulate the on-ramp merging problem as an Markov decision process (MDP). The input state information is the camera image data from the road side unit (RSU) and BSM data from the vehicles. This multi-modal information is trained on the reinforcement learning (RL) framework to train the ego vehicle making a merge to the highway. Further, we propose a reward function which is the feedback given to the policy. 

In summary, the contributions of this paper are as follows:-
\begin{itemize}
    \item We build a gym based SUMO environment for taper type  and parallel type merge lane. We introduce a multi-stage reward function which considers safety, comfort and traffic efficiency. We consider a  reward function before the merging intersection which finds the optimal gap to merge and driving comfort. Further a separate reward function which additionally considers collision and traffic congestion once the merging vehicle is on the highway.    
    \item Control decisions are made from the partial information from the image and BSM data. We add noise to the image data to simulate bad weather conditions. Additionally we add noise to the BSM data to demonstrate inaccurate sensor measurements
\item 
\end{itemize}

This paper is organized as follows. Section \ref{RelatedWork} reviews the related work and recent progress in this topic. In Section \ref{sec:ProbleStatement}, we mathematically formulate the problem and show the environment we are considering to solve the problem. In Section \ref{sec:Experiments} we run the experiments to show the working of our approach. 



In summary, the contributions of this paper are as follows:
\begin{itemize}
\item We propose a robust on-ramp merging approach named RMMRL to reliably handle the complicated and potential noisy driving environments. RMMRL jointly takes driving safety, comfort driving behavior, and traffic efficiency into account.
%By taking key characteristics of on-ramp merging tasks, we formulate the on-ramp merging problem as an MDP. Besides, a multi-stage reward function is introduced to handle the complicated merging considerations, where the driving safety, comfort driving behavior, and traffic efficiency are jointly taken into account. We introduce a multi-stage reward function which considers safety, comfort and traffic efficiency. We consider a  reward function before the merging intersection which finds the optimal gap to merge and driving comfort. Further a separate reward function which additionally considers collision and traffic congestion once the merging vehicle is on the highway.    

\item In order to solve the merging problem, we model the environment on the SUMO platform. We add augment the input observations using random scaling and Gaussian blur.  %To enable robust merging, we develop a augMented Multi-modal and  Reinforcement Learning  (RMMRL) approach using PPO.
%\item To enable robust merging, we develop a multi-modal and augmented reinforcement learning approach using PPO.  %Control decisions are made from the partial information from the image and BSM data. We add noise to the image data to simulate bad weather conditions. Additionally we add noise to the BSM data to demonstrate inaccurate sensor measurements

\item Extensive experiments are conducted by using Simulation of Urban MObility (SUMO) platform.
% We build a gym based SUMO environment for taper type and parallel type merge lane. First, We compare our proposed RMMRL model with the baseline approach defined by the SUMO's car following model and RL based single modality models. We achieve $47\%$ lower merge time, while $5\%$ change in driving comfort. Further, we validate the effectiveness of our augmented multi-modal design by extensive tests in variety of noisy observations. Lastly, we demonstrate the generalizability in taper-type and parallel-type merging scenarios.
\end{itemize}

==> Chapters/archive/Plan.tex <==
\section{Plan}

\begin{itemize}

    \item \textbf{Compare the proposed policy with the baseline approaches:}
    We will be considering two car-following model as the baseline to compare it with our approach.Average returns (total rewards per episode) for N(300) episodes for the experiments should be more than the baselines.
        \begin{enumerate}
            
            \item \textbf{Krauss Baseline Model} The baseline is run on the same reward function on the same environment as the proposed policy with a difference that the ego vehicle controlled by the SUMO's default Krauss car following model.
            \item \textbf{Imperfect Baseline Model} We compare our proposed policy with another baseline model with imperfection with simulated imperfect driving behavior.
        \end{enumerate}

    \item \textbf{Effect of imperfection of observation data} 
    \begin{enumerate}
        \item The information from the BSM data could be inaccurate. For example the GPS data accuracy is 3 meter. We add noise to the position of the vehicle to account for this inaccuracy in the measurements.
    \end{enumerate}
    \item \textbf{Partial image Information}
    \begin{enumerate}
        \item It is not always possible to get the image of the complete road segment. We consider the subsection of road segment at the intersection of 50 meters before and after the merge point. Further we will train of the BSM+noise data and compare this proposed policy with the baseline models from SUMO. 
    \end{enumerate}
    \item \textbf{Design different losses for the PPO network}
        \item 
    The degree of the noise and the impact of the noise on the approach. We can discuss that.may be now or in the future work.
    We can consider we have the two types of source data and both of them cannot be accurate, 
    WE can site sakets work 
    
    image nosie
    
    figure three after bsm + image then 
    bsm only and image only with noise
    rewards without noise is not required 
    
  
  
 figure 1
 
    baselines  
    
    bsm and image in the one figure
    
 figure 2
 
    bsm   

    bsm + noise and image
    
figure 3

    image  
    
    image+ noise and bsm
    
    
level of the noise impact 

or diff loss functions in the ppo model



To do
Implement the loss functions from the end to end imiation learning

re weight the wait function 

we have


figure of the final result, number of collusion and the total completion time


decompose the rewards


Just show them the perspective of safety and efficiency



Edit figure 2 showing the loop of the experiments
how the inut is generated how stable base lines which create the figure


we can add more things in the figure if have diff loss functions. 
 One more MGDA 
 we just consider equal contribution of equal source. 
 Consider diff ratios,
 
 two ways multiple 
 Highlight during the training
 consider diff sizes of the image
 
 
 no need for the captions and number of steps below the line and 
 normalize rewards value on te
 
 traingin we can have noise and while testing 
 
 
 
 x axis is regrading the noise
 
 
 trainign we have 4 models
 
 perfect bsm and perfect image Started
 
    - compare it with single model perfect image and perfect bsm
 add noise image and noise to bsm to augment the model 
  - since we augument our approach dont 
 
 train on parallel type lane only one type of new perfect bsm and image 
 
 
 training we have bsm only and image only and bsm + image
 
 
 testing
 
 with diff types of data.
 noisy data and check the models performance on the noise level. noise extreme level just random 

 


models 

BSM + No image
Image + No Bsm 
BSM+Image
BSMNoise + ImageNoise 




Revise the table 1 and table to compare it with bsm + no image, image + no bsm 

Round of 4 decimal
number of collisions as average . 

table 2 at diff noise levels compare. 


Parallel training use the same setting as taper type. For all of the training. 

Table 1 should be fair comparison. with the same number of episodes, batch size, etc. 

Section 5. Discussions on augmented reinforcement learning. add one paragraph to summarise the paper in comments . 





Add a figure to show a parallel type design.


\end{itemize}

==> Chapters/archive/ReinforcementLearning.tex <==
Reinforcement learning (RL) learns the policy function by mapping the states to actions through interactions with the environment. First, the agent takes actions based on the current state of the environment, which transitions the environment to the next state. Then the environment gives feedback to the agent in the form of a numerical reward and the next state. Based on these rewards, the RL algorithm updates the policy. This process continues until the agent learns to take preferred actions by maximizing the rewards.  

Reinforcement learning can be classified into model-based and model-free methods \cite{sutton2018reinforcement}. Model in this context is the model of the environment which predicts the behavior of the environment. It is how an environment will react by taking certain actions. If the model is known then the policy that agent follows can be found directly \cite{deepRL-2020}. Usually, the environment is stochastic and model of the environment is unknown. In such cases model-free method are used in which agent learns the policy by interacting with the black box environment. Model free can be further classified into value based methods and policy based methods. Value based methods are sample efficient but difficult to optimize for stable behavior \cite{nachum2017bridging,deepRL-2020}. Policy based methods are suitable for continuous action spaces and and have better convergence. J Schulman \textit{et. al.} introduced a model-free policy optimization method called Trust Region Policy Optimization (TRPO) \cite{schulman2015trust}. TRPO updates the policy with a constraint on the size of the update \cite{schulman2017proximal}. The surrogate objective function is defined as:
\begin{align}
    \underset{\theta}{maximize} \ L_{\theta_{old}} \left( \theta \right) \\
    s.t. \ D_{KL}^{max} \left( \theta_{old},\theta)  \right) \leq \delta,
\end{align}
where $\theta$ is the network parameters for the policy $\pi_{\theta} \left( a|s) \right)$, and $\theta_{old}$ are the parameters of the old policy. This policy is updated on the trust region constraint of  KL divergence denoted by $D_{KL}$ ,where $\delta$ is the bound on KL divergence \cite{schulman2015trust}.

PPO uses a clipped surrogate objective which is a modification of of the objective of the TRPO network. The network is trained to get maximize the expected returns from the loss function \cite{schulman2017proximal}:
\begin{equation}
    L_t^{CLIP + VF + S} \left( \theta \right) = \hat{\mathbb{E}_t} \left[ L_t^{CLIP} \left( \theta \right) - c_1 L_t^{VF} \left( \theta \right)  + c_2 S_{\left[ \pi_{\theta} \left( s_t \right) \right]} \right],
\end{equation}
where c1, c2 are coefficients and S denotes the entropy bonus, $L_t^{CLIP}$ is the clipped objective, second term $L_t^{VF} \left( \theta \right) $ is the Mean Squared error between the value function and the target value function, and the third term gives entropy bonus. The individual losses are defined as :
\begin{equation} \label{eq:PPO_loss}
     L_t^{CLIP} \left( \theta \right) = \hat{\mathbb{E}_t} \left[ min\left( r_t(\theta)  \hat{A_t},  clip\left( r_t(\theta) , 1- \epsilon, 1+ \epsilon \right) \right)\right],
\end{equation}
where
\begin{equation}
    r_t(\theta) = \frac{\pi_{\theta}\left(a_t, s_t\right)}{\pi_{\theta_{old}}(a_t, s_t)},
\end{equation}
where $\epsilon$ is a coefficient, $\hat{A_t}$ is the advantage function \cite{schulman2017proximal}. 

We chose PPO network because of its simpler policy parameterization, and better convergence in continuous and high dimensional action spaces.

==> Chapters/archive/State_Space_2.tex <==
 The highway section is shown in ~Fig. \ref{fig:mergingScenario}. For successful merging, an ego vehicle needs information on its own state and the states of other vehicles on the highway~\cite{nishitani2020deep}. Consider an ego vehicle at time step $t$ travels with velocity $v_{ego}$ and acceleration of $acc_{ego}$ at position $p_{ego}$. Hence, the state of the ego vehicle is defined as $S_{ego} = [v_{ego}, p_x ,p_y, acc_{ego}]$, where $p_x$ and $p_y$ are $x$ and $y$ coordinates of the ego vehicle's position. Vehicles on the highway upload their information to the RSU through BSM. The BSM consists of the current location and velocity of the vehicles~\cite{nuthalapati2016reliability,cowlagi2021Risk}. Similarly, we define the state information of the other vehicles in lanes 1 and 2. Besides, the roadside surveillance camera can capture the traffic conditions that inherently incorporate vehicles' driving behaviors and the highway traffic topology. The surveillance image will be sent to the RSU and then delivered to the ego vehicle~\cite{wen2019high}. Hence, the state of vehicles on the highway is defined as a dictionary object by, 
\begin{equation}
    S = \{ S_{ego}, S_1, S_2 , img \},
\end{equation}
where $S_{ego}, S_1, S_2 $ are the states of ego vehicle, and vehicles in lane 1 and lane 2 respectively. In each sub-state, vehicle velocity $v$, position $p_x, p_y$, and acceleration $acc$ are recorded. Additionally, the $img$ is the surveillance image from the RSU.
Thus the state information consists of two parts, BSM data $S_{ego}, S_1, S_2 \in \mathbb{R}^4$ and image data $img \in [0,255]^{W \times H \times C}$, where $W, H, C $ are the width, height and number of channels respectively.
